Toward Physically Realizable Quantum Neural Networks

There has been significant recent interest in quantum neural networks (QNNs), along with their applications in diverse domains. Current solutions for QNNs pose significant challenges concerning their scalability, ensuring that the postulates of quantum mechanics are satisfied and that the networks are physically realizable. The exponential state space of QNNs poses challenges for the scalability of training procedures. The no-cloning principle prohibits making multiple copies of training samples, and the measurement postulates lead to non-deterministic loss functions. Consequently, the physical realizability and efficiency of existing approaches that rely on repeated measurement of several copies of each sample for training QNNs are unclear. This paper presents a new model for QNNs that relies on band-limited Fourier expansions of transfer functions of quantum perceptrons (QPs) to design scalable training procedures. This training procedure is augmented with a randomized quantum stochastic gradient descent technique that eliminates the need for sample replication. We show that this training procedure converges to the true minima in expectation, even in the presence of non-determinism due to quantum measurement. Our solution has a number of important benefits: (i) using QPs with concentrated Fourier power spectrum, we show that the training procedure for QNNs can be made scalable; (ii) it eliminates the need for resampling, thus staying consistent with the no-cloning rule; and (iii) enhanced data efficiency for the overall training process since each data sample is processed once per epoch. We present a detailed theoretical foundation for our models and methods' scalability, accuracy, and data efficiency. We also validate the utility of our approach through a series of numerical experiments.

==> NN.tex <==
\begin{figure}[htp]
\centering
\begin{tikzpicture}[
plain/.style={
  draw=none,
  fill=none,
  },
net/.style={
  matrix of nodes,
  nodes={
    draw,
    circle,
    inner sep=8.5pt
    },
  nodes in empty cells,
  column sep=0.6cm,
  row sep=-11pt
  },
>=latex
]
\matrix[net] (mat)
{
|[plain]| \parbox{1cm}{\centering Input\\layer} & |[plain]| \parbox{1cm}{\centering Hidden\\layer} & |[plain]| \parbox{1cm}{\centering Output\\layer} \\
& |[plain]| \\
|[plain]| & \\
& |[plain]| \\
|[plain]| & |[plain]| \\
& & \\
|[plain]| & |[plain]| \\
& |[plain]| \\
|[plain]| & \\
& |[plain]| \\
};
\foreach \ai [count=\mi ]in {2,4,...,10}
  \draw[<-] (mat-\ai-1) -- node[above] {I\mi} +(-1cm,0);
\foreach \ai in {2,4,...,10}
{\foreach \aii in {3,6,9}
  \draw[->] (mat-\ai-1) -- (mat-\aii-2);
}
\foreach \ai in {3,6,9}
  \draw[->] (mat-\ai-2) -- (mat-6-3);
\draw[->] (mat-6-3) -- node[above] {O1} +(1cm,0);
\end{tikzpicture}

\caption{ANN diagram for Speed Sign recognition.}
\label{fig_m_3}
\end{figure}

==> QFourier.tex <==


%\subsection{Preliminaries}
\label{subsec:QFoureir}
\paragraph{Basic Definitions:} We can add the usual definitions here: Quantum states, density operators, POVM
{\bf ayg: this needs to be completed.}

\paragraph{Quantum Fourier Expansions for Operators on Qubits:} The standard Fourier expansion on the Boolean cube can be used to express any real-valued and bounded function on $\pmm^d$ as:
$$f(\bfx)=\sum_{S\subseteq [d]} \fS \pS(\bfx),$$  where $\pS(\bfx)=\prod_{j\in \mathcal{S}} x_j$ and $\fS=\EE_{\sim Unif}[f(\bfX) \pS(\bfX)]$. 
 %For the quantum counterpart, the \textit{Pauli} operators are used as the basis. Let $H_d\equiv (\CC^2)^{\tensor n}$ denote the Hilbert space of $d$ qubits.   
The quantum analog of the Boolean Fourier expansion is based on  \textit{Pauli} operators, together with the identity. These operators are denoted as: $\{\sigma^0,\sigma^1, \sigma^2, \sigma^3\}$. 
%% and characterized in the standard basis as
%{  \begin{align*}
% \sigma^0 & =  \begin{pmatrix}
% 1 & 0\\ 0 & 1
% \end{pmatrix}
%&   \sigma^1 &= \begin{pmatrix}
% 0 & 1\\ 1 & 0
% \end{pmatrix}\\
%\sigma^2 & =  \begin{pmatrix}
% 0 & -i\\ i & 0
% \end{pmatrix}
%&  \sigma^3 &=  \begin{pmatrix}
% 1 & 0\\ 0 & -1
% \end{pmatrix}.
% \end{align*}  }
%It is well-known that any Hermitian operator on $H_1$ can be uniquely written as a linear combination of the Pauli operators with real coefficients. Therefore, based on Pauli operators, one can develop a Fourier expansion for bounded operators  on $H_d$, the Hilbert space of $d$ qubits. In what follows, we give an overview of this expansion as presented in \citep{Montanaro2008}.  

%We first present a \textit{noncommutative} analog of correlation between random variables, which is an important concept in ordinary probability theory. Let $\rho$ be a fixed density operator acting on the Hilbert space  $H_d$. Consider the following inner product between any bounded operators $A, B$:
%\begin{align}\label{eq:Q inner prod}
%\<A,B\>_\rho \deq \tr\{A^\dagger B \rho\}.
%\end{align}
%It is easy to see that $\<A,B\>_\rho$ is a valid \textit{complex inner product}. Further, when $\rho$ is maximally mixed (i.e., $\rho= \frac{1}{2^d}\id$), then this inner product is equivalent to the normalized Hilbert-Schmidt inner product. 
%
%%Let us use the inner product defined in \eqref{eq:Q inner prod} with $\rho$ being maximally mixed, hence the normalized Hilbert-Schmidt inner product. 
%Going back to quantum Fourier development, it is not difficult to check that for $d=1$, the Pauli operators are orthonormal. For $d>1$, we create an orthonormal basis by \textit{tensoring} the Pauli operators. For that define, 
%%\vspace{-5pt}
%\begin{align}\label{eq:Pauly for s}
%\sigma^{\bfs}\equiv \sigma^{s_1}\tensor \sigma^{s_2}\tensor \cdots \tensor \sigma^{s_d}, \qquad \forall \bfs\in \{0,1,2,3\}^d.
%\end{align}
%When $\rho$ is maximally mixed, by construction, these operators are orthonormal, that is for any $\bfs,\bft\in \set{0,1,2,3}^d$, $\bfs\neq \bft$ the following equalities hold:
%$$
%\<\qps, \sigma^\bft\>_\rho=\prod_{j=1}^d \tr{\sigma^{s_j}\sigma^{t_j}}=0,\qquad \<\qps,\qps\>_\rho=1.$$
%Further, the set of all $\sigma^{\bfs}$ for $\bfs\in \{0,1,2,3\}^d$ forms an orthonormal basis for bounded operators on $H_d$. More formally, we obtain the Fourier expansion below. 
%\addva{
%\begin{proposition}\label{prop:quantum Fourier}
%Any bounded  operator $A$ on $H_d$ can be uniquely written as   $A = \sum_{\bfs \in \{0,1,2,3\}^d} a_{\bfs} ~\sigma^{\bfs},$ where $a_\bfs\in \CC$ are the Fourier coefficients of $A$ \addvb{and are given as $a_\bfs=\frac{1}{2^d}\tr\big\{A\qps\big\}$.} 
%\end{proposition}
%
%}
\begin{remark}[Quantum Fourier Expansions on qubits]\label{rem:quantum Fourier}
Any bounded  operator $A$ on the Hilbert space of $d$ qubits can be uniquely written as:   $A = \sum_{\bfs \in \{0,1,2,3\}^d} a_{\bfs} ~\sigma^{\bfs},$ where $a_\bfs\in \CC$ are the Fourier coefficients of $A$ {and are given by $a_\bfs=\frac{1}{2^d}\tr\big\{A\qps\big\}$.} If $A$ is Hermitian then $\qas \in \RR$. 
\end{remark}


==> backup.tex <==
It is not difficult to check that the expected outcome of $\mathcal{N}$ gives  $\Delta \Loss$ as in \eqref{eq:Delta Loss}:
\begin{align*}
\tr{(\Lambda_1-\Lambda_{-1}) V_\bfs^\dagger \tilde{\rho}_1 V_\bfs}& = \frac{1}{2} \tr{ \ketbra{0}_1 e^{-i\epsilon \qps}  \rho^{out}_1  e^{i\epsilon \qps}}\\
&+\frac{1}{2}\tr {\ketbra{1}_1 e^{i\epsilon \qps}  \rho^{out}_1  e^{-i\epsilon \qps}}\\
&-\frac{1}{2} \tr{ \ketbra{0}_1 e^{i\epsilon \qps}  \rho^{out}_1  e^{-i\epsilon \qps}}\\
&-\frac{1}{2}\tr {\ketbra{1}_1 e^{-i\epsilon \qps}  \rho^{out}_1  e^{i\epsilon \qps}}\\
&=\Delta\Loss(\overrightarrow{a}\pm \epsilon_\bfs,y_1)
\end{align*}
Hence, from \eqref{eq:Delta Loss}, the derivative of the loss is estimated using repeated measurements with $\mathcal{N}$ and dividing the results by $2\epsilon$.


\subsection{SGD for the expected empirical loss}
We start with explaining SGD for the relaxed assumption that exact copies of each sample is available. In that case, by repeated measurements one can compute $\Loss(\overrightarrow{a}, \rho_j, y_j)$. 


For SGD, we start with the first sample $(\rho_1, y_1)$.  
Since the samples are unknown, we won't be able to calculate the right-hand side. Instead, by measuring identical copies of the samples, we estimate the above quantity.




\paragraph{Measuring the gradient of the loss:}
 In what follows, we explain the procedure for measuring the derivative of the expected loss. The procedure is depicted in Figure \ref{fig:QNN gradient}. Instead of approximating the derivative using the finite difference method, we exactly coalculate it using a similar method introduced in \cite{Mitarai2018}.  For that, we first apply the QNN on $\rho_1$ that produces $\rho_1^{out}$. Next, we add an auxiliary qubit to $\rho^{out}_1$ that creates the following state
 \begin{align*}
 \tilde{\rho}_1 = \rho^{out}_1 \tensor \ketbra{+}_E,
 \end{align*}
 where $\ket{+}_E=\frac{1}{\sqrt{2}}(\ket{0}_E+\ket{{1}}_E)$, and $E$ represents the auxiliary Hilbert space. Then, we apply the following unitary operator on $\tilde{\rho}_1$
 \begin{align*}
 V_\bfs =  e^{i\epsilon \qps} \tensor \ketbra{0}_E + e^{-i\epsilon \qps} \tensor \ketbra{1}_E.
 \end{align*}
The resulted state state will be 
\begin{align*}
V_\bfs^\dagger \tilde{\rho}_1 V_\bfs  =  \frac{1}{2}\Big(& e^{-i\epsilon \qps}  \rho^{out}_1  e^{i\epsilon \qps} \tensor \ketbra{0}\\
& + e^{-i\epsilon \qps}  \rho^{out}_1  e^{-i\epsilon \qps} \tensor \outerproduct{0}{1}\\
& + e^{i\epsilon \qps}  \rho^{out}_1  e^{i\epsilon \qps} \tensor \outerproduct{1}{0}\\
& + e^{i\epsilon \qps}  \rho^{out}_1  e^{-i\epsilon \qps} \tensor \outerproduct{1}{1}\Big).
\end{align*}

\begin{figure}[hbtp]
\centering
\includegraphics[scale=1.1]{GradientQNN.eps}
\caption{The procedure for measuring the sub-gradient of the loss. A unitary operator $V_\epsilon$ followed by a quantum measurement $\mathcal{N}$ is used to measure the gradient of the loss at the current parameters of the network. The outcome of this measurement is a random variable $Z$ whose expectation equals to the gradient of the loss.}
\label{fig:QNN gradient}
\end{figure}


Then, we measure this state using $\mathcal{N}:=\set{\Lambda_{-1}, \Lambda_{1}}$ with outcomes in $\pmm$ and operators
\begin{align*}
\Lambda_{-1}  = \ketbra{0}_1 \tensor \ketbra{1}_E + \ketbra{1}_1 \tensor \ketbra{0}_E,\\\numberthis \label{eq:Measurement N}
\Lambda_{1}  = \ketbra{0}_1 \tensor \ketbra{0}_E + \ketbra{1}_1 \tensor \ketbra{1}_E.
\end{align*}
It is not difficult to check that the expected outcome of $\mathcal{N}$ gives  $\Delta \Loss$ as in \eqref{eq:Delta Loss}:
\begin{align*}
\tr{(\Lambda_1-\Lambda_{-1}) V_\bfs^\dagger \tilde{\rho}_1 V_\bfs}& = \frac{1}{2} \tr{ \ketbra{0}_1 e^{-i\epsilon \qps}  \rho^{out}_1  e^{i\epsilon \qps}}\\
&+\frac{1}{2}\tr {\ketbra{1}_1 e^{i\epsilon \qps}  \rho^{out}_1  e^{-i\epsilon \qps}}\\
&-\frac{1}{2} \tr{ \ketbra{0}_1 e^{i\epsilon \qps}  \rho^{out}_1  e^{-i\epsilon \qps}}\\
&-\frac{1}{2}\tr {\ketbra{1}_1 e^{-i\epsilon \qps}  \rho^{out}_1  e^{i\epsilon \qps}}\\
&=\Delta\Loss(\overrightarrow{a}\pm \epsilon_\bfs,y_1)
\end{align*}
Hence, from \eqref{eq:Delta Loss}, the derivative of the loss is estimated using repeated measurements with $\mathcal{N}$ and dividing the results by $2\epsilon$.
 


% For that, taking the derivative of the loss with respect to $\qas$ gives
%\begin{align*}
%\frac{\partial  \Loss( \overrightarrow{a}, y_1)}{\partial \qas} &= \frac{i\qas}{2}y_1\tr{(M_1-M_0)  \qps  U_1(\overrightarrow{a})^\dagger\rho_1 U_1(\overrightarrow{a})}\\
%& - \frac{i\qas}{2}y_1\tr{(M_1-M_0)    U_1(\overrightarrow{a})^\dagger \rho_1 \qps U_1(\overrightarrow{a})}\\
%&= \qas y_1 \Im\Big[\tr{(M_1-M_0)    U_1(\overrightarrow{a})^\dagger \rho_1 \qps U_1(\overrightarrow{a})}\Big]
%\end{align*}
%This derivative can be estimated by repeated measurements on exact copies of the samples.
 Consequently, the SGD is obtained at each time $t$ by the following rule: 
\begin{align*}
\overrightarrow{a}^{(t+1)} = \overrightarrow{a}^{(t)} - \eta_t \nabla \Loss( \overrightarrow{a}, y_t)
\end{align*}
After $T$ iterations, we set $\overrightarrow{a}=\frac{1}{T}\sum_t \overrightarrow{a}^{(t)}$ as the final update.
 

\subsection{SGD without exact copy}
Now we assume that only one copy of each sample is available and sample reuse is prohibited. In this case,  the expected loss $\Loss$ in \eqref{eq:expected loss} and its gradient are unknown. Furthermore, the training states $\rho_i$ are unknown with no exact copy available. We show that the procedure depicted in Figure \ref{fig:QNN gradient} is still applicable to this case. 

The idea is to apply the measurement $\mathcal{N}$  as in \eqref{eq:Measurement N} on $\Vs^\dagger (\rho^{out}\tensor \ketbra{+}) \Vs$ and to multiply the outcome by the true label $y$. At each time $t$, denote the result by $Z_t$. Note that $Z_t$ is a random variable depending on the current parameters of the network and the input sample  $(\rho_t, y_t)$.  

\begin{lem}
$Z_t$ gives an unbiased estimation of the derivative of the loss. More precisely,  
\begin{align*}
\EE[Z_t|y_t, \rho_t] = 2\epsilon \frac{\partial \Loss(\overrightarrow{a},y_1)}{\partial \qas}+O(\epsilon^2)
\end{align*}
\end{lem}
\begin{align*}
\EE[Z_t|y_t, \rho_t] & = y_t \tr{(\Lambda_1-\Lambda_{-1}) \Vs^\dagger (\rho_t^{out}\tensor \ketbra{+}) \Vs} \\
&=\Delta\Loss(\overrightarrow{a}\pm \epsilon_\bfs,y_1)\\
&= 2\epsilon \frac{\partial \Loss(\overrightarrow{a},y_1)}{\partial \qas}+O(\epsilon^2),
\end{align*}
where the last equality follows form \eqref{eq:Delta Loss}.
Continuing this process for all $\bfs$'s, we get a random vector $\overrightarrow{Z}_t$ whose expected value gives the gradient of the loss, that is $\EE[\overrightarrow{Z}_t| \rho_t, y_t] = 2\epsilon \nabla \Loss(\overrightarrow{a},\rho_t, y_t)+O(\epsilon^2).$ This implies that $\overrightarrow{Z}_t$ is a random vector (in the sub-gradient) that gives an unbiased estimate of the gradient.  
